A Fixed-Point Approach for Causal Generative Modeling

We propose a novel formalism for describing Structural Causal Models (SCMs) as fixed-point problems on causally ordered variables, eliminating the need for Directed Acyclic Graphs (DAGs), and establish the weakest known conditions for their unique recovery given the topological ordering (TO). Based on this, we design a two-stage causal generative model that first infers in a zero-shot manner a valid TO from observations, and then learns the generative SCM on the ordered variables. To infer TOs, we propose to amortize the learning of TOs on synthetically generated datasets by sequentially predicting the leaves of graphs seen during training. To learn SCMs, we design a transformer-based architecture that exploits a new attention mechanism enabling the modeling of causal structures, and show that this parameterization is consistent with our formalism. Finally, we conduct an extensive evaluation of each method individually, and show that when combined, our model outperforms various baselines on generated out-of-distribution problems. The code is available on \href{https://github.com/microsoft/causica/tree/main/research_experiments/fip}{Github}.

==> sections/cgm.tex <==
\subsection{Causal Generative Model}
\label{sec:cgm}
We are now ready to present our causal generative model to learn fixed-point SCMs from observational data. Given a dataset $\mathcal{D}$, we use our amortized TO predictor $\mathcal{M}$ to infer in a zero-shot manner the TO and use its prediction to learn $\mathcal{T}_{\text{ANM}}$ by minimizing~\eqref{eq:MSE-training} where $P$ is inferred by $\mathcal{M}(\mathcal{D})$.
% and we learn the function $\mathcal{T}_{\text{ANM}}$ to fit the dataset $\mathcal{D}$ by minimizing 
% $$
% \mathbb{E}_{\bm{X}\sim \hat{\mathbb{P}}_{\bm{X}}}
% \Vert \bm{X} - \textbf{CGM}(\mathcal{D})(\bm{X},0_d)\Vert_2\; .
% $$



==> sections/overview.tex <==
\section{Overview and Problem Set Up}
\label{sec:overview}
\textbf{Structural Causal Models.} Given a tuple $(\bm{f},\mathbb{P}_{\bm{N}})$, an SCM describes a data-generating process
that transforms a set of $d$ exogenous and independent random variables, $\bm{N}\sim\mathbb{P}_{\bm{N}}$, into a set of $d$ (observed) endogenous
random variables, $\bm{X}$, according to $\bm{f}$. Specifically, the SCM $\mathcal{S}(\bm{f},\mathbb{P}_{\bm{N}})$  generates the endogenous variables as follows:
\begin{align}
    \label{eq:scm-simplified}
    X_i = f_i(\textbf{PA}(X_i),N_i),~\quad \forall i\in\{1,\dots,d\}
\end{align}
where $\bm{X} := [X_1,\dots,X_d]$, $\bm{N}:=[N_1,\dots,N_d]$ and $\bm{f}:=[f_1,\dots,f_d]$. Each $i$-th component of $\bm{f}$ maps the $i$-th exogenous variable $N_i$ to the $i$-th endogenous
variable $X_i$, given the subset of the endogenous variables that directly cause $X_i$, i.e. the parents of $X_i$ ($\textbf{PA}(X_i)$)\footnote{Refer to Appendix~\ref{sec:background} for a complete definition.}. The equations introduced in~\eqref{eq:scm-simplified} depend implicitly on a graph that indicates the parents of each endogenous variable. This graph is assumed to be directed and acyclic\footnote{Refer to Appendix~\ref{sec:background} for formal defintions.}. For such graphs, it is always possible to order the nodes in a specific manner. More formally, there exists a permutation $\pi$, that is a bijective mapping  $\pi: \{1,\dots, d \}  \to \{1,\dots, d \}, $ satisfying $\pi(i) < \pi(j)$ if $j$ is a parent of $i$. We call such a permutation a topological ordering of the graph and it does not have to be unique. In the following we denote $\Sigma_d$ the set of permutation matrices of size $d$, and $\mathbb{P}_{\bm{X}}$ the distribution of $\bm{X}$. 

\CZ{Can we bring more foundation model setting or true world model thougts in. This has been discussed many time before}
\begin{figure}[!t]
\centering
\includegraphics[width=.9\linewidth]{figures/fig_causal.pdf}
\caption{Simplified scheme of the proposed approach.\label{fig:simplified-scheme}}
\end{figure}

\textbf{Problem Set Up.} \CZ{There are all standard set up. Do we want to discuss that there is a true world model and observations are different sub-graphs etc here? Is this a good place to connect to any foundation model settings?} Let us now introduce the problem of interest in this paper. Given $n$ i.i.d samples $\mathcal{D}:=\{\bm{X}^{(1)},\dots,\bm{X}^{(n)}\}$ drawn from a distribution $\mathbb{P}_{\bm{X}}$ generated by an unknown SCM $\mathcal{S}(\bm{f},\mathbb{P}_{\bm{N}})$, our goal is to recover the generating SCM from the observations $\mathcal{D}$.

% $\mathcal{S}(\bm{\tilde{f}},\mathbb{P}_{\bm{\tilde{N}}})$ that can explain these observations, i.e. generate $\mathbb{P}_{\bm{X}}$. Finding $\mathcal{S}(\bm{f},\mathbb{P}_{\bm{N}})$ would be sufficient to solve our task, however we cannot guarantee in general the identifiability of such models as there might exist several SCMs that can generate the same observational distribution $\mathbb{P}_{\bm{X}}$. \CZ{Does the last sentence belong to the problem set up?}

% \textbf{Learning an SCM is Hard.} One major limitation when it comes to parametrize an SCM is that the functional relationships $\bm{f}$ introduced in~\eqref{eq:scm-simplified} implicitly depend on an \emph{unknown} DAG which lives in a discrete space that grows super-exponentially w.r.t the number of variables. 


\CZ{Is this the right place for this? Also, this is just the fix point view not the full framework}
\textbf{Proposed Approach.}  In order to address this problem, we propose a new formalism to define SCMs viewed as fixed-point problems that do not require any DAGs. Based on our new definition, we then decompose the learning of the SCM into two steps: we propose first to infer in a zero-shot manner a topological ordering $\hat{\pi}$ from the data $\mathcal{D}$, and then to learn a generating SCM $\hat{\mathcal{S}}$ explaining the observations from the data $\mathcal{D}$ and the predicted topological ordering $\hat{\pi}$. See Figure~\ref{fig:simplified-scheme} for an illustration of the method. 

\CZ{I think that we should have a solution overview somewhere which cover the whole framework (section 3,4,5). Also the advantages of the solution should come across much more clear in section 1, 2 and around the solution overview. Currently, the advantages are not sold}

% \textbf{Outline.} In section~\ref{sec:scm}, we introduce our new and equivalent formalism to define an SCM viewed as a fixed point problem. We also provide partial identifiability results (i.e. when we also have access to the topological ordering) of these models in two important cases. In section~\ref{sec:topological}, we present the methodology adopted to train in a amortized manner our topological ordering predictor at scale from observations only. In section~\ref{sec:scm_learning}, we present our new attention-based architecture that aims at inferring the full SCM generating the data when both the observations and the topological ordering are given. In \ref{sec:cgm}, we present our final causal generative model that aims at inferring the full generating SCM from observational data only. Finally in section~\ref{sec:experiments}, we investigate the performances of our proposed approach on various complex experiments.




==> sections/transistion_scm.tex <==
Next, we present how we move progressively from the standard representation of SCMs to the proposed fixed-point parameterization that does not require DAGs.

\subsection{Standard SCMs as Fixed-Point Problems}
From the standard definition of SCMs, one can obtain an equivalent fixed-point formulation by reparameterizing the functional relationships. 

Let us define 
$F^{\mathcal{G}}:\mathbb{R}^d\times \mathbb{R}^d\to \mathbb{R}^d$, satisfying $\forall i\in\{1,\dots,d\},~~x,n\in\mathbb{R}^d$:
\begin{align*}
F_i^{\mathcal{G}}(x,n):= F_i(x_{\text{pa}_1(i)},\dots,x_{\text{pa}_{\textit{c}_i}(i)},n_i),
\end{align*}
where $F^{\mathcal{G}}(x,n):=[F_1^{\mathcal{G}}(x,n),\dots,F_d^{\mathcal{G}}(x,n)]$, $x:=[x_1,\dots, x_d]$, $n:=[n_1,\dots, n_d]$, and for all $i$, $(\text{pa}_1(i),\dots,\text{pa}_{c_i}(i))$ is the sequence of parents of $i$ in $\mathcal{G}$ ranked in the increasing order and $c_i$ the number of parents of $i$ in $\mathcal{G}$. Observe that here, we have made explicit the dependence between $F^{\mathcal{G}}$ and the graph $\mathcal{G}$, as  each $F^{\mathcal{G}}_i$ is the composition of the function $F_i$ with the operator $\textbf{PA}_{\mathcal{G}}^{(i)}(x):=[x_{\text{pa}_1(i)},\dots, x_{\text{pa}_{\textit{c}_i}(i)}]\in \mathbb{R}^{c_i}$ that projects $x\in\mathbb{R}^d$ into the coordinates given by the parents of $i$ in $\mathcal{G}$. Then the assignments introduced in~\eqref{eq:scm-simplified} can be equivalently reformulated as the following fixed-point problem on $\bm{X}$:
\begin{align}
\label{eq:scm_fp}
\bm{X}=F^{\mathcal{G}}(\bm{X},\bm{N}).
\end{align}
In the following, we denote $\mathcal{S}_{\text{eq}}(\mathbb{P}_{\bm{N}},F^{\mathcal{G}})$ the reparameterized standard SCM associated to $\mathbb{P}_{\bm{N}}$ and $F^{\mathcal{G}}$.

% In the following Proposition, we show that this reparameretization is equivalent to the standard formulation.
% \begin{proposition}
% There exists a bijection between $\mathcal{S}$ and $\mathcal{S}_{\text{eq}}$, and we denote such equivalence relation as $\mathcal{S}\longleftrightarrow \mathcal{S}_{\text{eq}}$.
% \end{proposition}

Therefore, by applying this reparameterization on the functional relationships, we obtain an equivalent representation of standard SCMs as fixed-point problems. However, the functional relationships $F^{\mathcal{G}}$ involved in the fixed-point problem~\eqref{eq:scm_fp} still depends on a DAG $\mathcal{G}$. As a first step towards removing this dependency, we propose next to augment this equivalent representation of SCMs with TOs.

% We will see in the following that by augmenting the representation of standard SCMs with a topological ordering, we obtain a new representation that is independent of DAGs.

\subsection{An Augmented Represention of Standard SCMs}

Here we aim at obtaining a representation of SCMs that is able to distinguish between two same standard SCMs when ordered with two different topological orderings. More formally, given a reparametrized  standard SCM $\mathcal{S}_{\text{eq}}( \mathbb{P}_{\bm{N}}, F^{\mathcal{G}})$, and two valid topological orderings (if they exist) $\pi_1\neq \pi_2$ associated to $\mathcal{G}$, we want to be able to distinguish between $\mathcal{S}_{\text{eq}}( \mathbb{P}_{\bm{N}}, F^{\mathcal{G}})$  when ordered according to $\pi_1$ with the same SCM $\mathcal{S}_{\text{eq}}( \mathbb{P}_{\bm{N}}, F^{\mathcal{G}})$ when ordered according to $\pi_2$.

To do so, we propose to simply augment the previous representation of standard SCMs by adding to the parameterization a valid topological ordering. Let $\pi$ a topological ordering associated to the DAG $\mathcal{G}$ and let us define the 2-tuple $(\pi,\mathcal{S}_{\text{eq}}( \mathbb{P}_{\bm{N}}, F^{\mathcal{G}}))$ representing the augmented SCM with TO $\pi$. 
% Observe that this 2-tuple a simple augmentation of the previous representation of standard SCMs where we add a valid topological ordering into the parameterization. 
% Now, recall that for a given DAG, there (always exists at least one and) might exist multiple valid topological orderings. To clarify this, we denote $\Pi(\mathcal{G}):=\{\pi~\text{s.t.}~ \pi \text{ is a valid topological ordering of } \mathcal{G}\}$. Then, we define $\mathcal{S}_{\text{aug}}$, the set of all augmented SCMs, that is the set of all possible 2-tuples of the form $(\pi, \mathcal{S}_{\text{eq}}(\mathbb{P}_{\bm{N}},F^{\mathcal{G}}))$ with $\pi\in\Pi(\mathcal{G})$. 
While this augmented representation does not remove the dependency between the functional relationship $F^{\mathcal{G}}$ and the graph $\mathcal{G}$, it has the essential advantage to enable distinguishing between two same standard SCMs but endowed with two different topological orderings, a property that does not enjoy the standard formulation of SCMs. 

In the following, we leverage this property of augmented SCMs and present a reparameterization that induces a simple structure on the functional relationships.

\subsection{Augmented SCMs as Fixed-Point Problems on the Ordered Nodes}
% In this section, we leverage the topological ordering of the augmented representation to define a new fixed-point on the ordered nodes. 

Let $(\pi, S_{\text{eq}}(\mathbb{P}_{\bm{N}},F^{\mathcal{G}}))$ an augmented SCM, and let us denote $P_{\pi}\in\Sigma_d$ the permutation matrix associated to the topological ordering $\pi$. Then by defining $F_{\pi}^{\mathcal{G}} \colon \mathbb{R}^d\times  \mathbb{R}^d  \to \mathbb{R}^d$ such that for all $x,n\in\mathbb{R}^d$ 
\begin{equation}
\label{eq:func_ordered}
\begin{gathered}
F_{\pi}^{\mathcal{G}}(x,n):=\\
[F_{\pi^{-1}(1)}^{\mathcal{G}}(P_\pi^{T} x, P_\pi^{T} n),\dots,F_{\pi^{-1}(d)}^{\mathcal{G}}(P_\pi^{T} x, P_\pi^{T} n)],
\end{gathered}
\end{equation}
we obtain an equivalent formulation of~\eqref{eq:scm_fp} defined as the following fixed-point problem on $\bm{X}$: 
\begin{align}
\label{eq:fp_ordered}
\bm{X}=P_{\pi}^TF_\pi^{\mathcal{G}}(P_{\pi}\bm{X}, P_\pi\bm{N}).
\end{align} 
Observe that we have made explicit the dependence of the function $F_\pi^{\mathcal{G}}$ with both the graph $\mathcal{G}$ and the TO $\pi$, due to its definition. 
% In the following we denote $\mathcal{S}_{\text{fp}}(P_\pi,\mathbb{P}_{\bm{N}},F_{\pi}^{\mathcal{G}})$ such reparameterization of augmented SCM.
% and $\mathcal{S}_{\text{fp}}$ the set of all possible $\mathcal{S}_{\text{fp}}(P_\pi,\mathbb{P}_{\bm{N}},F_{\pi}^{\mathcal{G}})$. 
% Let us now show the equivalence between $\mathcal{S}_{\text{fp}}$ and $\mathcal{S}_{\text{aug}}$.
% \begin{proposition}
% $\mathcal{S}_{\text{aug}}$ is in bijection with $\mathcal{S}_{\text{fp}}$, that is $\mathcal{S}_{\text{aug}}\longleftrightarrow\mathcal{S}_{\text{fp}}$.
% \end{proposition}
The main advantage of this reparameterization is that now $F_\pi^{\mathcal{G}}$ must satisfy a simple structure.
\begin{lemma}
\label{lem-existence-fp-paper}
Let $F_\pi^{\mathcal{G}}$ as defined in~\eqref{eq:func_ordered}, then it satisfies for all $x,n\in\mathbb{R}^d$:
\begin{equation*}
\begin{aligned}
[Jac_1 F_\pi^{\mathcal{G}}(x,n)]_{i,j} &= 0,\quad \text{if}\quad j\geq i,\quad \text{and} \\ 
[Jac_2 F_\pi^{\mathcal{G}}(x,n)]_{i,j} &= 0,\quad \text{if}\quad i\neq j,
\end{aligned}
\end{equation*}
where $\textnormal{Jac}_1 F_\pi^{\mathcal{G}}$ and $\textnormal{Jac}_2 F_\pi^{\mathcal{G}}$ are the Jacobians of $F_\pi^{\mathcal{G}}$ w.r.t the first and second variables, i.e. $x$ and $n$ respectively.
\end{lemma}

Thus, the function $F_\pi^{\mathcal{G}}$, defining the fixed-point problem~\eqref{eq:fp_ordered} on the ordered nodes, has to admit a strictly lower-triangular Jacobian w.r.t $x$ and a diagonal Jacobian w.r.t $n$. While $F_\pi^{\mathcal{G}}$ still has a dependency with the graph $\mathcal{G}$ (as well as the topological odering $\pi$), we show in the following section that the condition of Lemma~\ref{lem-existence-fp-paper} is also sufficient to parameterize the augmented SCMs, enabling the introduction of a new formalism to define them independently of DAGs.


% However, we still have a dependency between the functional relationship $F_\pi^{\mathcal{G}}$, and the graph $\mathcal{G}$ (as well as the topological odering $\pi$). 


% We now ask the following question: 
% \begin{question}
% Is the above condition on the functions sufficient to remove the dependency with DAGs in their parameterization? 
% \end{question} 

% In the following, we answer this question in the affirmative and present our new definition of fixed-point SCMs that does not require DAGs.

